MA-RLHF: Reinforcement Learning from Human Feedback with Macro Actions

Reinforcement learning from human feedback (RLHF) has demonstrated effectiveness in aligning large language models (LLMs) with human preferences. However, token-level RLHF suffers from the credit assignment problem over long sequences, where delayed rewards make it challenging for the model to discern which actions contributed to preferred outcomes. This hinders learning efficiency and slows convergence.In this paper, we propose MA-RLHF, a simple yet effective RLHF framework that incorporates macro actions -- sequences of tokens or higher-level language constructs -- into the learning process. By operating at higher level of abstraction, our approach reduces the temporal distance between actions and rewards, facilitating faster and more accurate credit assignment. This results in more stable policy gradient estimates and enhances learning efficiency within each episode, all without increasing computational complexity during training or inference. We validate our approach through extensive experiments across various model sizes and tasks, including text summarization, dialogue generation, question answering, and program synthesis. Our method achieves substantial performance improvements over standard RLHF, with performance gains of up to 30% in text summarization and code generation, 18% in dialogue, and 8% in question answering tasks. Notably, our approach reaches parity with vanilla RLHF 1.7 ~ 2 times faster in terms of training time and continues to outperform it with further training. We make our code and data publicly available at https://github.com/ernie-research/MA-RLHF.

==> section/analysis_old.tex <==
\subsubsection{Scaling Experiments on Summarize}
\label{appendix:tl;dr_scaling}


    % \begin{minipage}{0.30\linewidth}
    % \centering
    % \includegraphics[width=1.0\columnwidth]{figure/scaling.pdf}
    % \captionsetup{type=figure} \vskip -1em
    % \caption{Scaling trend when evaluated by RM, GPT-4, and Human. }
    % \label{fig:tl;dr-scaling}
    % \end{minipage}

\begin{figure}
\centering
\includegraphics[width=0.3\columnwidth]{figure/tl;dr_27B_main.pdf}
\includegraphics[width=0.3\columnwidth]{figure/tl;dr_27B_rm_distribution.pdf}
\includegraphics[width=0.34\columnwidth]{figure/scaling.pdf}
\caption{\textcolor{brown}{Evaluation results for vanilla PPO and MA-PPO on Gemma-2-27B using the TL;DR dataset. \textbf{Left} RM scores on validation set. \text{Mid} distribution of RM scores for vanilla PPO and MA-PPO. \text{Right} scaling trending on TL;DR dataset across 2B, 7B, and 27B model size, with RM scores, GPT-4 evaluation, Human evaluation results.}}
\label{fig:scaling}
\end{figure}

\textcolor{brown}{We verify the effectiveness of MA-PPO on the Gemma-2-27B model. As shown in \Cref{fig:scaling} (Left and Mid), MA-PPO consistently exhibits superior performance compared to vanilla PPO, and shows a remarkable pattern on obtaining a higher reward scores. In \Cref{fig:scaling} (Right), we demonstrate the scaling trend of MA-PPO across 2B, 7B, and 27B models, involving RM score, GPT-4 evaluation, and human evaluation results. These results indicate the effectiveness and scalability of MA-PPO.}


\subsubsection{Macro Action Selection}
\label{sec:analysis-ma-selection}

\begin{figure}
\centering
\begin{minipage}{0.63\linewidth}
    \centering
    \includegraphics[width=0.48\textwidth]{figure/tl;dr_2B_varying_k.pdf}
    \includegraphics[width=0.48\textwidth]{figure/dialogue_2B_varying_k.pdf}
    \caption{Test RM scores of different $n$ in MA-PPO evaluated by corresponding reward model of Gemma-2B model on the TL;DR (Left) and HH-RLHF (Right) dataset.}
    \label{fig:analysis_vary_k}
\end{minipage}
\hspace{2.5mm}
\begin{minipage}{0.32\linewidth}
    \includegraphics[width=1.0\textwidth]{figure/tl;dr_fine_grained_score.pdf}
    \caption{GPT-4 scores of vanilla PPO and MA-PPO with different $n$ settings on TL;DR. }
    \label{fig:fine_grained_score}
\end{minipage}
\end{figure}

\begin{figure}[t]
\centering
\begin{minipage}{0.48\linewidth}
\centering
\includegraphics[width=\columnwidth]{figure/MA-RLHF-selection.pdf}
\caption{Illustration of four option selections in MA-RLHF framework. Each selection outputs a list of $\ell(\tau)$. In the parsing based selection, the macro action is determined when the tokens number of current node is less than $C=5$, which is represented as number in tree node.}
\label{fig:selection_illustration}
\end{minipage}
\hspace{1mm}
\begin{minipage}{0.48\linewidth}
\includegraphics[width=0.48\textwidth]{figure/tl;dr_2B_selection.pdf}
\includegraphics[width=0.48\textwidth]{figure/tl;dr_selection_fine_grained_score.pdf}
\caption{Performance of MA-PPO with different macro action selections on TL;DR dataset for Gemma-2B model. \textbf{Left} test RM scores. \textbf{Right} GPT-4 scores across 4 dimensions.}
\label{fig:analysis_selection}
\end{minipage}
\end{figure}

\begin{figure}[t]
\centering
\begin{minipage}{0.48\linewidth}
\centering
\includegraphics[width=0.8\columnwidth]{figure/MA-RLHF-value-function.pdf}
\caption{Illustration of value function of macro actions in MA-RLHF framework. It takes the outputs from the value function of tokens as input, and returns the value of macro actions with different $\sigma_\tau$ assignment.}
\label{fig:value_function_illustration}
\end{minipage}
\hspace{1mm}
\begin{minipage}{0.48\linewidth}
\includegraphics[width=0.48\textwidth]{figure/tl;dr_2B_implementation.pdf}
\includegraphics[width=0.48\textwidth]{figure/tl;dr_implementation_score.pdf}
\caption{Performance of MA-PPO with different weight vector in MA-PPO on TL;DR dataset for Gemma-2B model. \textbf{Left} test RM scores. \textbf{Right} GPT-4 scores on 4 dimensions.}
\label{fig:analysis_implementation}
\end{minipage}
\end{figure}

% \begin{table*}[t]
% \begin{minipage}{0.40\linewidth}
% \scriptsize
% \caption{Pass@$k$ ($k=\{1,5\}$) metric evaluated on the APPS test set.}
% \scalebox{0.75}{
% \begin{tabular}{c|c|cc|cc}
% \toprule
% \multicolumn{2}{l|}{\multirow{2}{*}{Method}} & \multicolumn{2}{c|}{2B} & \multicolumn{2}{c}{7B} \\
% \cmidrule(lr){3-6}
% \multicolumn{2}{l|}{}                        & PPO       & MA-PPO     & PPO       & MA-PPO     \\
% \midrule
% \multirow{4}{*}{pass@1} & Inter. & 2.82      & $\textbf{3.25}_{\textcolor{deepgreen}{\text{+15\%}}}$       & 4.26      & $\textbf{6.22}_{\textcolor{deepgreen}{\text{+46\%}}}$       \\
%                         & Intro. & 15.26     & $\textbf{16.56}_{\textcolor{deepgreen}{\text{+8\%}}}$      & 20.90     & $\textbf{26.74}_{\textcolor{deepgreen}{\text{+28\%}}}$      \\
%                         & Comp.  & 0.92      & $\textbf{0.94}_{\textcolor{deepgreen}{\text{+2\%}}}$       & 1.21      & $\textbf{2.00}_{\textcolor{deepgreen}{\text{+65\%}}}$       \\
%                         & All    & 4.92      & $\textbf{5.45}_{\textcolor{deepgreen}{\text{+11\%}}}$       & 6.98      & $\textbf{9.48}_{\textcolor{deepgreen}{\text{+35\%}}}$       \\
% \midrule
% \multirow{4}{*}{pass@5} & Inter. & 4.10      & $\textbf{4.37}_{\textcolor{deepgreen}{\text{+7\%}}}$       & 6.57      & $\textbf{8.37}_{\textcolor{deepgreen}{\text{+27\%}}}$       \\
%                         & Intro. & 17.30     & $\textbf{18.30}_{\textcolor{deepgreen}{\text{+6\%}}}$      & 23.30     & $\textbf{30.30}_{\textcolor{deepgreen}{\text{+30\%}}}$      \\
%                         & Comp.  & \textbf{1.70}      & $1.60_{\textcolor{brown}{\text{-6\%}}}$       & 2.30      & $\textbf{3.30}_{\textcolor{deepgreen}{\text{+43\%}}}$       \\
%                         & All    & 6.26      & $\textbf{6.60}_{\textcolor{deepgreen}{\text{+5\%}}}$       & 9.06      & $\textbf{11.74}_{\textcolor{deepgreen}{\text{+30\%}}}$    \\
% \bottomrule
% \end{tabular}
% }
% \label{tab:apps_results}
% \end{minipage}
% \centering
% \begin{minipage}{0.45\linewidth}
% \captionsetup{type=figure} \vskip -1em
% \centering
% \subfigbottomskip=-5pt
% \subfigure[Macro Action Selection]{
% \includegraphics[width=0.48\textwidth]{figure/tl;dr_2B_selection.pdf}
% \includegraphics[width=0.48\textwidth]{figure/tl;dr_selection_fine_grained_score.pdf}
% \label{fig:analysis_selection}
% }
% \\
% \subfigure[Macro Action Value Function]{
% \includegraphics[width=0.48\textwidth]{figure/tl;dr_2B_implementation.pdf}
% \includegraphics[width=0.48\textwidth]{figure/tl;dr_implementation_score.pdf}
% \label{fig:analysis_implementation}
% }
% \caption{Performance of MA-PPO under different settings on TL;DR dataset.}
% \end{minipage}
% \end{table*}
In this section, we delve into option selection in MA-RLHF, a key factor in modeling macro actions. While the $n$-gram based selection was the primary method due to its effectiveness and adaptability, we introduce additional selections illustrated in \Cref{fig:selection_illustration}.

\textbf{Macro Action Length of $n$-gram Based Selection$\:$} In fixed $n$-gram based selection, a hyper-parameter $n$ is used to control the macro action length. In this section, we investigate the performance of MA-RLHF with different choices of $n$, where $n\in\{3,5,10,\infty\}$. The experiments are conducted on the TL;DR and HH-RLHF datasets, with RM scores of validation set are shown in \Cref{fig:analysis_vary_k}. We find that all choices of $n$ lead to performance improvements. Notably, $k=\infty$ achieves the best performance on the TL;DR dataset, while $n=10$ perform best on the HH-RLHF dataset.

% To further understand the strengths and weaknesses of MA-PPO with varying macro action length, we utilize GPT-4 to score the generated summaries across 4 criteria: relevance, coherence, consistency, and fluency, as we did in the pairwise comparison in Section~\ref{sec:tl;dr_results}. However, unlike the previous evaluation, GPT-4 assigns scores to each summarization individually for each criteria. The relevance, coherence, and consistency scores range from 0 to 7, while fluency is rated from 0 to 5. 
The GPT-4 scores are presented in \Cref{fig:fine_grained_score}. Although MA-PPO with $n=5$ does not achieve the best performance under the reward model evaluation (\Cref{fig:analysis_vary_k}), it consistently outperforms vanilla PPO across all criteria. The $n=3$ and $n=10$ configurations also achieve notable scores in relevance, coherence, and consistency, but do not surpass vanilla PPO in fluency. Interestingly, modeling the whole sequence as a macro action (\emph{i.e.}, $n=\infty$) negatively impacts coherence and fluency.


\textbf{Macro Action Selections: } We utilize RM score and GPT-4 estimated score to estimate the performance of macro action selections. In \Cref{fig:analysis_selection} (Left), we report the RM score. Despite the selections of macro action are different, all of which outperform vanilla PPO. Notably, both fixed and dynamic $n$-gram based selections achieve the best performance after training on half of the total samples. In \Cref{fig:analysis_selection} (Right), we presents GPT-4 scores on four criteria. As expected, perplexity based selection significantly improves fluency, while dynamic $n$-gram based selection performs best on the other criteria. 

\subsubsection{Value Function Estimation of Macro Action}
\label{sec:analysis-ma-implementation}
% \begin{figure}
% \centering
% \includegraphics[width=0.39\textwidth]{figure/tl;dr_2B_implementation.pdf}
% \hspace{5mm}
% \includegraphics[width=0.40\textwidth]{figure/tl;dr_implementation_score.pdf}
% \caption{Performance of MA-PPO with different weight vector in MA-PPO on TL;DR dataset for Gemma-2B model. \textbf{Left} presents test reward scores evaluated by RM. \textbf{Right} shows the GPT-4 scores on 4 dimensions.}
% \label{fig:analysis_implementation}
% \end{figure}

When implementing the macro actions, the value function of macro actions is estimated through the value function of tokens. This process can be formulated as: $V^\pi(s_\tau,\omega_\tau) = \sum_{i=0}^{\ell(\tau)}\sigma_{t_{\tau}+i}V^\pi(s_{t_\tau+i},a_{t_\tau+i})$, where $\sigma_{\tau}=\{\sigma_{t_\tau},\cdots,\sigma_{t_\tau+\ell(\tau)}\}$ control the contribution of each value function of tokens.

% \begin{equation}
% \label{eqn:value_function_of_ma}
%     V^\pi(s_\tau,\omega_\tau) = \mathbb{E}\left[\sigma_{t_\tau}V^\pi(s_{t_\tau},a_{t_\tau})+\cdots+\sigma_{t_\tau+\ell(\tau)+1}V^\pi(s_{t_\tau+\ell(\tau)+1},a_{t_\tau+\ell(\tau)+1})\right]
% \end{equation}


In this section, we explore several assignments of $\sigma_\tau$ and their effectiveness on MA-PPO. \Cref{fig:value_function_illustration} illustrates macro action value function with different $\sigma_\tau$ assignments: (a) \textbf{Equal assignment}: We treats the contributions of each value function of tokens equally when considering the value function of macro actions. This is the naive assignment in MA-PPO used in all our experiments. (b) \textbf{Unit assignment}: Since a macro action is a higher-level construct of a sequence of actions, we can use the value function of the last action as the macro action’s value function. (c) \textbf{Position decayed assignment}: The contributions of each value function of tokens are determined by taking the position into consideration. We refer to Appendix~\ref{appendix:value-function} for implementation details.

We tested these approaches with fixed $n$-gram based selection on TL;DR dataset, with $n=5$. We report the RM score and GPT-4 score as previous. Results in \Cref{fig:analysis_implementation} show that the all ones weight vector yields higher RM scores. However, the unit weight vector achieves the best consistency and fluency according to GPT-4 evaluations.

\subsubsection{Impact of RLHF on Temperature}

\begin{figure}
    \centering
    \includegraphics[width=0.24\textwidth]{figure/tl;dr_sft_bon.pdf}
    \includegraphics[width=0.24\textwidth]{figure/tl;dr_ppo_bon.pdf}
    \includegraphics[width=0.24\textwidth]{figure/tl;dr_ma-ppo_bon.pdf}
    \caption{Impact of temperature on RM score when sampling N outputs.  \textbf{Left} mean RM score of the SFT model under different temperature and sampling sizes (N). \textbf{Mid} mean RM score of vanilla PPO. \textbf{Right} mean RM score of MA-PPO.}
    \label{fig:analysis_temperature_bon}
\end{figure}

\textbf{Best-of-$N$ (rejection sampling)} improves response quality by selecting the highest-reward response from $N$ samples generated by the policy model. We evaluate MA-PPO, SFT, and vanilla PPO with best-of-$N$ sampling across temperature $t\in\{0.2, 0.4, 0.6, 0.8, 1.0, 1.2\}$ and sample sizes $N\in\{4,8,16,32\}$. In \Cref{fig:analysis_temperature_bon}, we observe that best-of-$N$ sampling improves RM scores for all methods, with higher $N$ yielding better results. SFT and vanilla PPO are sensitive to temperature, requiring adjustments for optimal performance. In contrast, MA-PPO is more robust, consistently performing best at $t = 1.2$, with improvements across all temperatures except for best-of-4.

We also observe that MA-PPO maintains stable performance across different sampling temperature settings, as detailed in Appendix~\ref{appendix:analysis_temperature}.

\subsubsection{Impact of RLHF on Reward Score Distribution}
\begin{figure}
    \centering
    \includegraphics[width=0.22\textwidth]{figure/tl;dr_rm_score_shift_bon.pdf}
    \includegraphics[width=0.22\textwidth]{figure/tl;dr_rm_score_shift_vanilla-ppo.pdf}
    \includegraphics[width=0.22\textwidth]{figure/tl;dr_rm_score_shift_ma-ppo.pdf}
    \includegraphics[width=0.22\textwidth]{figure/tl;dr_rm_score_shift_ma-ppo-infty.pdf}
    \caption{RM score shifting pattern after RLHF training.  \textbf{Left} presents the RM score of best of 8 sampling compared to the SFT. \textbf{Mid} presents the RM score of vanilla PPO compared to the SFT model. \textbf{Right} presents the RM score of MA-PPO (n=5 and n=$\infty$ compared to the SFT model.}
    \label{fig:analysis_rm_score_shift}
\end{figure}

In this section, we analyze the RM score shifting pattern after applying RLHF with vanilla PPO and MA-PPO on the TL;DR dataset. The RM scores of SFT model are taken as the baseline. We also include Best-of-$N$ sampling (with $N=8$) for the SFT model to illustrate the impact of RLHF. \Cref{fig:analysis_rm_score_shift} shows the normalized RM score shifting patterns. These results indicate that while Best-of-$N$ can enhance overall response quality, it is less effective than RLHF. Vanilla PPO moves the distribution towards higher score (upper left corner), but still leaves some low-quality long tail instances. In contrast, MA-PPO has a clearer positive impact on the distribution and reduce the number of low-quality long tail instances more effectively than vanilla PPO. 

\subsubsection{Effectiveness on Program Synthesis}

\begin{wraptable}{r}{0.39\textwidth}
\vspace{-4.5mm}
    \centering
    \scriptsize
    \caption{\label{tab:apps_results}Pass@$k$ ($k=\{1,5\}$) metric evaluated on the APPS test set.}
    \scalebox{0.75}{
    \begin{tabular}{c|c|cc|cc}
    \toprule
    \multicolumn{2}{l|}{\multirow{2}{*}{\textbf{Method}}} & \multicolumn{2}{c|}{\textbf{CodeGemma-2B}} & \multicolumn{2}{c}{\textbf{CodeGemma-7B}} \\
    \cmidrule(lr){3-6}
    \multicolumn{2}{l|}{}                        & \textbf{PPO}       & \textbf{MA-PPO}     & \textbf{PPO}       & \textbf{MA-PPO}     \\
    \midrule
    \multirow{4}{*}{pass@1} & Inter. & 2.82      & $\textbf{3.25}_{\textcolor{deepgreen}{\text{+15\%}}}$       & 4.26      & $\textbf{6.22}_{\textcolor{deepgreen}{\text{+46\%}}}$       \\
                            & Intro. & 15.26     & $\textbf{16.56}_{\textcolor{deepgreen}{\text{+8\%}}}$      & 20.90     & $\textbf{26.74}_{\textcolor{deepgreen}{\text{+28\%}}}$      \\
                            & Comp.  & 0.92      & $\textbf{0.94}_{\textcolor{deepgreen}{\text{+2\%}}}$       & 1.21      & $\textbf{2.00}_{\textcolor{deepgreen}{\text{+65\%}}}$       \\
                            & All    & 4.92      & $\textbf{5.45}_{\textcolor{deepgreen}{\text{+11\%}}}$       & 6.98      & $\textbf{9.48}_{\textcolor{deepgreen}{\text{+35\%}}}$       \\
    \midrule
    \multirow{4}{*}{pass@5} & Inter. & 4.10      & $\textbf{4.37}_{\textcolor{deepgreen}{\text{+7\%}}}$       & 6.57      & $\textbf{8.37}_{\textcolor{deepgreen}{\text{+27\%}}}$       \\
                            & Intro. & 17.30     & $\textbf{18.30}_{\textcolor{deepgreen}{\text{+6\%}}}$      & 23.30     & $\textbf{30.30}_{\textcolor{deepgreen}{\text{+30\%}}}$      \\
                            & Comp.  & \textbf{1.70}      & $1.60_{\textcolor{brown}{\text{-6\%}}}$       & 2.30      & $\textbf{3.30}_{\textcolor{deepgreen}{\text{+43\%}}}$       \\
                            & All    & 6.26      & $\textbf{6.60}_{\textcolor{deepgreen}{\text{+5\%}}}$       & 9.06      & $\textbf{11.74}_{\textcolor{deepgreen}{\text{+30\%}}}$    \\
    \bottomrule
    \end{tabular}
    }
\end{wraptable}

We evaluate the performance of MA-PPO on a program synthesis task. Due to the lack of reward model, we directly use the compiler signal as the final reward, following previous studies~\citep{ppocoder,rltf}. Implementation details can be found in Appendix~\ref{appendix:code}.
% \input{table/apps_results}

We compare the performance of MA-PPO and vanilla PPO using the pass@k (k=1,5) metric~\cite{codex} on the 5k test set from the APPS dataset. As demonstrated in Table~\ref{tab:apps_results}, MA-PPO achieve superior pass@k performance compared to vanilla PPO, particularly as model size increases. For 7B model, MA-PPO achieves +2.50 pass@1 and +2.68 pass@5 scores over vanilla PPO. 

\subsubsection{Advantages and State-Action Values of PPO}
We further analysis the advantages and state-action values of PPO during training to demonstrate the .

\begin{figure}[t]
    \centering
    \begin{minipage}{0.43\linewidth}
        \centering
        \includegraphics[width=1.0\columnwidth]{figure/tl;dr_advantages.pdf}
        \caption{\label{fig:tl;dr-advantages}Advantages of MA-PPO and vanilla PPO curves during training.}
    \end{minipage}
    \hspace{1.5mm}
    \begin{minipage}{0.43\linewidth}
        \centering
        \includegraphics[width=1.0\columnwidth]{figure/tl;dr_returns.pdf}
        \caption{\label{fig:tl;dr-returns}State-action values of MA-PPO and vanilla PPO curves during training.}
    \end{minipage}
\end{figure}



==> section/experiments_old.tex <==

\subsection{Summarization}
\label{sec:tl;dr_results}

As prior work notes, automatic metrics like ROUGE poorly correlate with human preferences~\citep{summarize_feedback,dpo}. We utilize the reward model, which scores the samples and is used to optimize the policy model during PPO training. The results are depicted in \Cref{fig:tl;dr-main}. We find that MA-PPO significantly improves summarization performance. Comparing to the references provided in the TL;DR validation set, both of the methods initially lag behind the references but rapidly surpass the references. 
\Cref{fig:tl;dr-rm-ditribution} illustrates a RM score shift of MA-PPO towards higher RM scores compared to vanilla PPO. 


Incorporating a superior LLM as a judge has been widely discussed in the field of LLMs~\citep{mt-bench}. To comprehensively estimate MA-PPO, we use GPT-4\footnote{The GPT-4 version is gpt-4o-05-13, and the temperature is set to 0.} to simulate the win-rate between MA-PPO and vanilla PPO.
% We employ GPT-4 to assess 50 samples selected from the 2k instances. To ensure the diversity of evaluation, the evaluated instances are selected based on the provided subreddit information and CNN Daily Mails. 
GPT-4 was presented with posts or articles with corresponding summarizations generated by different methods, and asked to select the preferred summarization based on four criteria: relevance, coherence, consistency, and fluency. To prevent bias, we randomized whether the summarization appeared as ``A'' or ``B'', as done in prior studies~\citep{DBLP:journals/corr/abs-2112-00861,mt-bench}. As shown in \Cref{fig:tl;dr-win-rate}, the responses generated by the MA-PPO are mostly preferred by GPT-4 for both model sizes. MA-PPO with Gemma-2B achieves 78\% win rate over vanilla PPO, and 86\% win rate with Gemma-7B model.

However, introducing GPT-4 as the judge can produce judge bias into the evaluation, which may prefers longer response when comparing responses~\citep{alpacaeval-2.0}. To mitigate this bias, we conduct a human evaluation on the same instances used in the GPT-4 evaluation, with the same procedure and criteria. Results shown in \Cref{fig:tl;dr-win-rate} indicate that MA-PPO still outperforms vanilla PPO with 74\% and 70\% win rate for the tested models.\footnote{To better illustrate the difference, we demonstrate some examples in Appendix~\ref{appendix:examples}.}

% \begin{table}
% \parbox{.45\linewidth}{
% \centering
% \begin{tabular}{ccc}
% \hline
% a&b&c\\
% \hline
% \end{tabular}
% \caption{Foo}
% }
% \hfill
% \parbox{.45\linewidth}{
% \centering
% \begin{tabular}{ccc}
% \hline
% d&e&f\\
% \hline
% \end{tabular}
% \caption{Bar}
% }
% \end{table}

% \begin{wraptable}{r}{0.39\textwidth}
%     \vspace{-5mm}
%     \centering
%     \scriptsize
% \begin{table}
%     \footnotesize
%     \parbox{.50\linewidth}{
%     \centering
%     % \scalebox{0.85}{
%      \caption{\label{tab:rm_score_and_ppl}RM scores of vanilla PPO and MA-PPO on TL;DR, HH-RLHF, and WebGPT datasets.} 
%     \begin{tabular}{l|lll}
%     \toprule
%     \textbf{Model}       & \textbf{TL;DR} & \textbf{HH-RLHF} & \textbf{WebGPT} \\
%     \midrule
%     Vanilla PPO (2B) & 0.84  & 1.31                        & -0.62                     \\
%     MA-PPO    (2B)    & $\textbf{1.41}_{\textcolor{deepgreen}{\text{+68\%}}}$  & $\textbf{1.55}_{\textcolor{deepgreen}{\text{+18\%}}}$                        & $\textbf{-0.60}_{\textcolor{deepgreen}{\text{+3\%}}}$                      \\
%     \midrule
%     Vanilla PPO (7B) & 1.90  & 1.05                        & -0.61                      \\
%     MA-PPO    (7B)    & $\textbf{2.47}_{\textcolor{deepgreen}{\text{+30\%}}}$  & $\textbf{1.24}_{\textcolor{deepgreen}{\text{+18\%}}}$                        & $\textbf{-0.56}_{\textcolor{deepgreen}{\text{+8\%}}}$                       \\
%     \bottomrule
%     \end{tabular}
%     }
%     \quad
%     \parbox{.50\linewidth}{
%     \centering
%     \caption{\label{tab:tl;dr-agreement}Agreement among reward model, GPT-4, and human evaluations on the TL;DR dataset.}
%     % \resizebox{0.35\textwidth}{!}{
%     \begin{tabular}{c|c|ccc}
%     \toprule
%         &  \textbf{\#Param}   & \textbf{RM}    & \textbf{GPT-4} & \textbf{Human} \\
%     \midrule
%     RM & \multirow{3}{*}{2B}   & 100\% & -     & -     \\
%                GPT-4  & & 78\%  & 100\% & -     \\
%                Human  & & 76\%  & 58\%  & 100\% \\
%     \midrule
%     RM     & \multirow{3}{*}{7B} & 100\% & -     & -     \\
%                GPT-4  & & 78\%  & 100\% & -     \\
%                Human  & & 74\%  & 64\%  & 100\% \\
%     \bottomrule
%     \end{tabular}
%     }

% \end{table}

\begin{table*}[t]
\centering
    \begin{minipage}{0.4\linewidth}
    \centering
    \small
    % \footnotesize
    \caption{\label{tab:tl;dr-agreement} Agreement among RM, GPT-4, and human evaluations on TL;DR.}
    \scalebox{0.85}{
    \begin{tabular}{c|c|ccc}
    \toprule
        &  \textbf{\#Param}   & \textbf{RM}    & \textbf{GPT-4} & \textbf{Human} \\
    \midrule
    RM & \multirow{3}{*}{2B}   & 100\% & -     & -     \\
               GPT-4  & & 78\%  & 100\% & -     \\
               Human  & & 76\%  & 58\%  & 100\% \\
    \midrule
    RM     & \multirow{3}{*}{7B} & 100\% & -     & -     \\
               GPT-4  & & 78\%  & 100\% & -     \\
               Human  & & 74\%  & 64\%  & 100\% \\
    \bottomrule
    \end{tabular}
    }
    \end{minipage}
\hspace{5mm}
    \begin{minipage}{0.55\linewidth}
    \centering
    % \footnotesize
    \small
     \caption{\label{tab:rm_score_and_ppl} Test RM scores of vanilla PPO and MA-PPO on TL;DR, HH-RLHF, and WebGPT datasets.} 
    \scalebox{0.9}{
    \begin{tabular}{l|lll}
    \toprule
    \textbf{Model}       & \textbf{TL;DR} & \textbf{HH-RLHF} & \textbf{WebGPT} \\
    \midrule
    Vanilla PPO (2B) & 0.84  & 1.31                        & -0.62                     \\
    MA-PPO    (2B)    & $\textbf{1.41}_{\textcolor{deepgreen}{\text{+68\%}}}$  & $\textbf{1.55}_{\textcolor{deepgreen}{\text{+18\%}}}$                        & $\textbf{-0.60}_{\textcolor{deepgreen}{\text{+3\%}}}$                      \\
    \midrule
    Vanilla PPO (7B) & 1.90  & 1.05                        & -0.61                      \\
    MA-PPO    (7B)    & $\textbf{2.47}_{\textcolor{deepgreen}{\text{+30\%}}}$  & $\textbf{1.24}_{\textcolor{deepgreen}{\text{+18\%}}}$                        & $\textbf{-0.56}_{\textcolor{deepgreen}{\text{+8\%}}}$                       \\
    \bottomrule
    \end{tabular}
    }
    \end{minipage}
\end{table*}



% \begin{wraptable}{r}{0.4\textwidth}
% \vspace{-5mm}
% \centering
% \scriptsize
% \caption{\label{tab:tl;dr-agreement}Agreement among reward model, GPT-4, and human evaluations on the TL;DR dataset.}
% \resizebox{0.35\textwidth}{!}{
% \begin{tabular}{c|c|ccc}
% \toprule
%     &  \textbf{\#Param}   & \textbf{RM}    & \textbf{GPT-4} & \textbf{Human} \\
% \midrule
% RM & \multirow{3}{*}{2B}   & 100\% & -     & -     \\
%            GPT-4  & & 78\%  & 100\% & -     \\
%            Human  & & 76\%  & 58\%  & 100\% \\
% \midrule
% RM     & \multirow{3}{*}{7B} & 100\% & -     & -     \\
%            GPT-4  & & 78\%  & 100\% & -     \\
%            Human  & & 74\%  & 64\%  & 100\% \\
% \bottomrule
% \end{tabular}}
% \end{wraptable}


We calculate the agreements among reward model, GPT-4, and human to assess the reliability of evaluating. Since the results of GPT-4 and human are pairwise, we calculate the win rate of reward model by selecting the summary with higher RM score. The agreements are presented in Table~\ref{tab:tl;dr-agreement}, showing that the reward model has a much higher agreement with both GPT-4 and humans. Additionally, the agreement between GPT-4 and human evaluators averaged 62\% across models, indicating the reliability of our evaluation methods.

% To comprehensively assess MA-PPO performance on LLMs, we conducted experiments on the Gemma-2-27B model using the TL;DR dataset. The performance trend is shown in Figure~\ref{fig:tl;dr-scaling} across 2B, 7B, and 27B models, involving RM score, GPT-4 evaluation, and human evaluation results, indicating the scalability of MA-PPO. More detailed results are shown in Appendix~\ref{appendix:tl;dr_scaling}.

\subsection{Single-Turn Dialogue} 

Next, we conduct experiments on the single-turn dialogue task using the Anthropic HH-RLHF dataset to evaluate performance in terms of helpfulness and harmlessness. The evaluation approaches are the same as the TL;DR evaluation. 

% \begin{figure}[t]
% \centering
% \begin{minipage}{0.60\linewidth}
%     \includegraphics[width=0.48\textwidth]{figure/dialogue_2B_main.pdf}
%     \includegraphics[width=0.48\textwidth]{figure/dialogue_7B_main.pdf}
%     \caption{Test RM scores evaluated by corresponding reward model of Gemma-2B and Gemma-7B model on HH-RLHF dataset.}
%     \label{fig:dialogue-main}
% \end{minipage}
% \hspace{1.5mm}
% \begin{minipage}{0.3\linewidth}
%     \centering
%     \includegraphics[width=0.97\columnwidth]{figure/dialogue_2B_rm_distribution.pdf}
%     \vspace{-3mm}
%     \caption{Distribution of test RM scores for vanilla PPO and MA-PPO on Gemma-2B using the HH-RLHF dataset. }
%     \label{fig:dialogue-rm-ditribution}
% \end{minipage}
% \hspace{1.5mm}
% \begin{minipage}{0.30\linewidth}
%     \centering
%     \includegraphics[width=1.0\columnwidth]{figure/dialogue_win_rate.pdf}
%     \caption{\label{fig:dialogue-win-rate}Win rates estimated by GPT-4 and Human with MA-PPO against vanilla PPO on the HH-RLHF dataset.}
% \end{minipage}
% \hspace{1.5mm}
% \begin{minipage}{0.35\linewidth}
%     \centering
%     \includegraphics[width=\columnwidth]{figure/qa_win_rate.pdf}
%     \vskip -0.6em
%     \caption{\label{fig:qa-win-rate}Win rates estimated by GPT-4 and Human with MA-PPO against vanilla PPO on the WebGPT Comparisons dataset.}
% \end{minipage}
% \vspace{-5mm}
% \end{figure}

%     \begin{minipage}{0.47\linewidth}
%         \centering
%         \footnotesize
%         \begin{tabular}{c|c|ccc}
%         \toprule
%  &    \#Param    & RM & GPT-4 & Human \\
%         \midrule
% RM & \multirow{3}{*}{2B} & 100\%        & -     & -     \\
%                     GPT-4        & & 56\%         & 100\% & -     \\
%                     Human        & & 52\%         & 50\%  & 100\% \\
%         \midrule
% RM & \multirow{3}{*}{7B} & 100\%        & -     & -     \\
%                     GPT-4       &  & 80\%         & 100\% & -     \\
%                    Human        &  & 60\%         & 64\%  & 100\% \\
%         \bottomrule
%         \end{tabular}
%         \caption{\label{tab:dialogue-agreement}Agreement among reward model, GPT-4, and human evaluations on HH-RLHF dataset.}
%     \end{minipage}

% The RM scores of different methods are listed in Figure~\ref{fig:dialogue-main}, showing a similar trend to the TL;DR experiments, where MA-PPO surpasses vanilla PPO after trained about 1/3 of the total training steps. 

For GPT-4 and human evaluation, we focus on the helpfulness criterion. The win rates are presented in \Cref{fig:dialogue-win-rate}, where models trained with MA-PPO consistently outperforms vanilla PPO. Notably, MA-PPO's win rate increases with model size. For models scaled from 2B to 7B, the GPT-4 win rate rises from 58\% to 72\%, while human evaluation win rates increase from 52\% to 60\%. This pattern also holds when using GPT-4 to evaluate the TL;DR dataset. More experimental results can be found in Appendix~\ref{appendix:exp_hh}.

% We calculate the agreements among three evaluation methods in Table~\ref{tab:dialogue-agreement}. However, we notice that the agreements of Gemma-2B model are not as correlated as the agreements under other cases. Still, the agreements of Gemma-7B model are showing the used metrics correlate with each other. We also find that the GPT-4 judgment correlate strongly with the trained reward model. 

\subsection{Question Answering}
We assess the performance of MA-PPO on the OpenAI WebGPT Comparison dataset, which focus on the question answering task. In \Cref{fig:qa-win-rate}, we present the evaluation results conducted by GPT-4 and Human, verifying the effectiveness of MA-PPO. More experiments on the question-answering tasks using the WebGPT dataset are detailed in Appendix~\ref{appendix:exp_webgpt}.

% \begin{wraptable}{r}{0.39\textwidth}
%     \vspace{-5mm}
%     \centering
%     \scriptsize
%     \caption{\label{tab:rm_score_and_ppl}RM scores of vanilla PPO and MA-PPO on TL;DR, HH-RLHF, and WebGPT datasets.}
%     \scalebox{0.85}{
%     \begin{tabular}{l|lll}
%     \toprule
%     \textbf{Model}       & \textbf{TL;DR} & \textbf{HH-RLHF} & \textbf{WebGPT} \\
%     \midrule
%     Vanilla PPO (2B) & 0.84  & 1.31                        & -0.62                     \\
%     MA-PPO    (2B)    & $\textbf{1.41}_{\textcolor{deepgreen}{\text{+68\%}}}$  & $\textbf{1.55}_{\textcolor{deepgreen}{\text{+18\%}}}$                        & $\textbf{-0.60}_{\textcolor{deepgreen}{\text{+3\%}}}$                      \\
%     \midrule
%     Vanilla PPO (7B) & 1.90  & 1.05                        & -0.61                      \\
%     MA-PPO    (7B)    & $\textbf{2.47}_{\textcolor{deepgreen}{\text{+30\%}}}$  & $\textbf{1.24}_{\textcolor{deepgreen}{\text{+18\%}}}$                        & $\textbf{-0.56}_{\textcolor{deepgreen}{\text{+8\%}}}$                       \\
%     \bottomrule
%     \end{tabular}
%     }
% \end{wraptable}

To provide a straightforward comparison, we list the RM scores of the final checkpoints in Table~\ref{tab:rm_score_and_ppl}. \textcolor{brown}{MA-PPO consistently achieves superior performance on three tasks, demonstrating the learning efficiency of MA-PPO. Specifically, the improvement on TL;DR is most outstanding since MA-PPO obtains 68\% and 30\% performance gain compared to vanilla PPO on 2B and 7B models. On the HH-RLHF and WebGPT datasets, MA-PPO consistently outperforms vanilla PPO with 18\% and 8\% improvements on 7B model.}


==> table/table_demo.tex <==
\begin{table}[!ht]
\caption{Sample table title}
\label{sample-table}
\begin{center}
\begin{tabular}{ll}
\multicolumn{1}{c}{\bf PART}  &\multicolumn{1}{c}{\bf DESCRIPTION}
\\ \hline \\
Dendrite         &Input terminal \\
Axon             &Output terminal \\
Soma             &Cell body (contains cell nucleus) \\
\end{tabular}
\end{center}
\end{table}



